RIOT: a Stochastic-based Method for Workflow Scheduling in the Cloud

Cloud computing provides engineers or scientists a place to run complex computing tasks. Finding a workflow's deployment configuration in a cloud environment is not easy. Traditional workflow scheduling algorithms were based on some heuristics, e.g. reliability greedy, cost greedy, cost-time balancing, etc., or more recently, the meta-heuristic methods, such as genetic algorithms. These methods are very slow and not suitable for rescheduling in the dynamic cloud environment. This paper introduces RIOT (Randomized Instance Order Types), a stochastic based method for workflow scheduling. RIOT groups the tasks in the workflow into virtual machines via a probability model and then uses an effective surrogate-based method to assess a large amount of potential scheduling. Experiments in dozens of study cases showed that RIOT executes tens of times faster than traditional methods while generating comparable results to other methods.

==> images/metrics.tex <==
\begin{figure}
    \centering
     \noindent
\begin{tikzpicture}[scale=0.7]

\begin{axis}[ axis x line=center,
  axis y line=center,
  ticks=none,
  xlabel={\Large $makespan$},
  ylabel={\Large $cost$},
  xlabel style={below right},
  ylabel style={above left},
  xmin=0.3,
  xmax=5,
  ymin=0.2,
  ymax=5]
  
\addplot [mark=none,domain=0.45:4.7] {1/ x*2.1};

\addplot[only marks] coordinates {
	(0.56,3.7)
	(0.7,3.0)
	(0.84,2.5)
	(1.4, 1.5)
	(3,0.7)
	(4.2,0.5)
};

\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (0.56,3.7) (1.0,4.5) };
\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (0.7,3.0) (1.4, 2.8) };
\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (0.84,2.5) (1.4, 2.8) };
\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (1.4, 1.5) (2.3, 1.5) };
\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (3,0.7) (3.6, 0.9) };
\addplot[no marks,  dashed, color=red, line width=2.5pt] coordinates { (4.2,0.5) (4.3, 0.8) };

	
\addplot [no marks,color = white, fill=black!20, fill opacity=0.65]coordinates {
	(1.0, 5.0)
    (1.0, 4.5)
    (1.4, 4.5)
	(1.4, 2.8)
	(2.3, 2.8)
	(2.3, 1.5)
	(3.6, 1.5)
	(3.6, 0.9)
	(4.3, 0.9)
	(4.3, 0.8)
	(4.5, 0.8)
	(4.5, 5.0)
};

\addplot[mark=square*, line width=1.0pt, dashed] coordinates {
	(1.0, 4.5)
	(1.4, 2.8)
	(2.3, 1.5)
	(3.6, 0.9)
	(4.3, 0.8)
	
};

\pgfplotsset{
    after end axis/.code={
        \node[black,above] at (axis cs:2.3,3.5){\Large{Hypervolume}};
        \node[black] at (axis cs:1.2,3.7){\Large{$d_1$}};
		\node[black] at (axis cs:1.9,2.2){\Large{$d_2$}};
		\node[black] at (axis cs:3.0,1.28){\Large{$\ldots$}};
		\node[black] at (axis cs:3.9,1.0){\Large{$d_n$}};
		
		\node[black] at (axis cs:0.8, 5.3){\Large{True frontier}};
		\node[black] at (axis cs:3.0, 5.1){\Large{Algorithm returns}};
    }
}

\addplot[no marks, color=black, line width=0.6pt, ->] coordinates { (0.3, 6.3) (0.5, 4.7) };
\addplot[no marks, color=black, line width=0.6pt, ->] coordinates { (3.3, 5.3) (1.2, 4.5) };
		
\end{axis}

\end{tikzpicture}
\caption{Illustration of performance metrics used in this paper. Hypervolume is a 
convergence and diversity indicator, filled in gray in this figure. Spread is the average
distance of consecutive objectives, i.e. $d_i$ shown in this figure.
IGD is average distance from solutions in true frontier to algorithm returns, i.e. {\color{red} red dashed
line} shown in this figure.
}
\label{fig:metrics}
\end{figure}


==> images/overhead.tex <==
 \begin{figure}[!t]
 \begin{tikzpicture}[scale=0.6]
 \pgfplotsset{every x tick label/.append style={font=\Large, yshift=0.5ex}}
\pgfplotsset{every y tick label/.append style={font=\Large, xshift=0.5ex}}
\begin{axis}[
	ymajorgrids,
        ybar,
    height=6cm,
    width=13cm,
    enlarge y limits=false,
    axis lines*=left,
    ymin=1,
    ymax=100,
	ymode=log,
	log ticks with fixed point,
	ytick={1,5,10,20, 40,100},
     legend style={at={(0.3, 1.2)},
        anchor=west,legend columns=-1},
        ylabel={\Large (opt+run)/run},
        symbolic x coords={medium6,medium1,medium5,medium4,medium3,large5,large4,medium2,large2,large1},
     xtick=data,
	 x tick label style={rotate=60,anchor=east}	 ]
\addplot +[
    black,
    fill=blue!30,
    postaction={
        pattern=north east lines
    }
]coordinates {(medium6,1.07) (medium1,1.17) (medium5,1.43) (medium4,1.71) (medium3,2.10) (large5,7.08) (large4,7.10) (medium2,9.28) (large2, 16.05) (large1,90.41)};
    \addplot [fill=red!80]coordinates {(medium6,1.00) (medium1,1.01) (medium5,1.02) (medium4,1.03) (medium3,1.02) (large5,1.45) (large4,1.21) (medium2,1.24) (large2, 1.63) (large1,4.95)};
    \legend{prior work, this work}
\end{axis}

 \end{tikzpicture}
 \caption{Overhead of optimization, measured as the fraction  $(\mathit{run} + \mathit{opt}) / \mathit{run}$  where $\mathit{run}$
 is the runtime of the optimized workflow and   $\mathit{opt}$  is the time required 
 to run the optimizer. {\em Medium*} and {\em Large*} are  workflows with $10^2$ and $10^3$ tasks, respectively.
 This table was generated using the case studies explored later in this paper.
 Workflows are sorted by the optimization overhead. }\label{fig:ab}
 \end{figure}

==> images/sampling.tex <==
\begin{figure*}[t!]
    \centering
     \noindent
    \begin{tabular}{cc}
    \setlength{\tabcolsep}{0.2em}
\begin{tikzpicture}[scale=1.0]

\pgfmathsetseed{1238}
\pgfmathsetseed{1238}
\pgfmathsetmacro{\c}{0.8}
\pgfmathsetmacro{\d}{1.2}
\fill [fill=black!5] (-2*\c,-1*\d) -- (7*\c, -1*\d) -- (7*\c, 1.5*\d) -- (-2*\c,1.5*\d) -- (-2*\c,-1*\d);

\fill [fill=black](0, 0) circle (0.07);
\node [text width=10pt] at (0, -0.3*\d) {$E_0$};

\fill [fill=black](5.8*\c, 0.7*\d) circle (0.07);
\node [text width=10pt] at (5.8*\c, 1.0*\d) {$E_1$};

\fill [fill=red](0.6*\c, 0.6) circle (0.07);
\node [text width=10pt] at (0.8*\c,0.88) {$C$};

% draw other anchors
\fill [fill=black!50](2.5*\c, -0.3*\d) circle (0.07);
\fill [fill=black!50](4.3*\c, 0.9*\d) circle (0.07);
\fill [fill=black!50](2.2*\c, -0.8*\d) circle (0.07);
\fill [fill=black!50](-0.3*\c, -0.8*\d) circle (0.07);
\fill [fill=black!50](-0.9*\c, 0.8*\d) circle (0.07);


\draw [dimen,dashed, every rectangle node/.style={fill=black!5, midway,font=\small}] (0,0) -- (5.8*\c,0.7*\d) node {$L$};
\draw (0,0) -- (-0.20*\c, 0.29*\d);
\draw (0.6*\c, 0.6*\d) -- (0.43*\c, 0.89*\d);
\draw [dimen,every rectangle node/.style={fill=black!5, midway,font=\small}] (-0.18*\c,0.26*\d) -- (0.42*\c, 0.88*\d) node {$l$};

% draw more anchors
\foreach \i in {1,...,3}{
\fill [fill=black!50](rand*2*\c+3.2*\c,rand*0.5*\d+0.5*\d) circle (0.07);
}


\node [text width=65] at (5.5*\c, -0.6*\d) {\Large
$\frac{l}{L}=\frac{O_0-\widehat{O}_{C}}{O_0-O_1}$};
\end{tikzpicture}
&

\begin{tikzpicture}[scale=1.0]


\pgfmathsetseed{123456}
\pgfmathsetmacro{\c}{0.8}
\pgfmathsetmacro{\d}{1.2}

\fill [fill=black!5] (-2*\c,-1*\d) -- (7*\c, -1*\d) -- (7*\c, 1.5*\d) -- (-2*\c,1.5*\d) -- (-2*\c,-1*\d);


\fill [fill=black](-0.9*\c, 0.8*\d) circle (0.07);
\node [text width=10pt] at (-0.7*\c, 1.1*\d) {$E_0$};

\fill [fill=black](5.8*\c, 0.7*\d) circle (0.07);
\node [text width=10pt] at (5.8*\c, 1.0*\d) {$E_1$};


\fill [fill=red](-1.7*\c, 0.36*\d) circle (0.07);
\node [text width=10pt] at (-1.7*\c, 0.68*\d) {$C$};

% draw other anchors
\fill [fill=black!50](4.8*\c, 0.7*\d) circle (0.07);
\fill [fill=black!50](3.4*\c, 1.3*\d) circle (0.07);
\fill [fill=black!50](4.3*\c, 0.9*\d) circle (0.07);
\fill [fill=black!50](2.2*\c, -0.8*\d) circle (0.07);
\fill [fill=black!50](0, 0) circle (0.07);
 
\draw [dimen,dashed, every rectangle node/.style={fill=black!5, midway,font=\small}] (-0.9*\c, 0.8*\d) -- (5.8*\c,0.7*\d) node {$L$};
\draw [dimen,every rectangle node/.style={fill=black!5, midway,font=\small}] (-1.7*\c, 0.36*\d) -- (-0.9*\c,0.8*\d) node {$l$};

% draw more anchors
\foreach \i in {1,...,2}{
\fill [fill=black!50](rand*2.3*\c+1.8*\c, rand*0.9*\d+0.3*\d) circle (0.07);
}

\node [text width=65] at  (5.5*\c, -0.6*\d) {\Large
$\frac{l}{L}=-\frac{O_0-\widehat{O}_{C}}{O_0-O_1}$};
\end{tikzpicture}


 \end{tabular}
    \caption{Estimating makespan(cost) of configuration $C$ ($\color{red} \bullet$) from known anchor configurations, marked by $\bullet$ or $\color{black!50} \bullet$.
    $E_0$, $E_1$ are nearest, furthest evaluated candidates to $C$. $O_0$ and $O_1$ are makespan(cost) of $E_0$ and $E_1$ respectively. $l$($L$) is the Manhattan distance between configurations of $C$ and $E_0$($E_1$).
    Formulations show the heuristic of objective-configuration relationships. Note that sign in RHS
    is determined by relative position of $C, E_0$ and $E_1$ (line 20 in Algorithm~\ref{alg:sample}).
    }
    \label{fig:sample_demo}

\end{figure*}


==> tables/relatedwork.tex <==
\newcommand\yes{\checkmark}
\newcommand\no{-}
\newcommand*\rot{\multicolumn{1}{R{30}{1.3em}}}% no optional argument here, please!
\newcolumntype{C}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{D}[1]{>{\centering\let\newline\\\arraybackslash\hspace{0pt}}m{#1}}
\newcolumntype{H}{>{\setbox0=\hbox\bgroup}c<{\egroup}@{}}
\definecolor{Gray}{gray}{0.85}

\begin{table}[!t]
\footnotesize

\caption{Highly Cited  Workflow Configuration Techniques from 2006 to present}
\centering
\setlength{\tabcolsep}{0.6em}
\begin{threeparttable}
\begin{tabular}{rccC{1.6cm}D{1.6cm}HHH}
%%%%%% HEADER%%%%%%
&\multicolumn{1}{c}{Author} & 
Cited by &
\multicolumn{1}{c}{\parbox{1.6cm}{\centering Optimization Strategy}} & 
% \multicolumn{1}{c}{\parbox{1.3cm}{\centering Evaluation\\Strategy}} &
% Ins Model\tnote{1} & 
%\parbox{1.3cm}{\centering VM Type\\Uniformity\tnote{2}} &
\multicolumn{1}{c}{Objectives}&
% \rot{\scriptsize Communication Cost Considered}&
% \rot{\scriptsize Optimization Overhead Analyzed}&
% \rot{\scriptsize Applied to Large Workflow\tnote{1}}&
% \rot{\scriptsize Adaptive\tnote{2}}&
&&
% \rot{\scriptsize Open Sourced}
\\\toprule

%%%%%%%%%% DATA
% \cite{topcuoglu2002performance}&Topcuoglu, 2002 & 1968 & HEFT & heuristic & limited & makespan & \yes& \no& \no& \no& \no\\
% \cite{he2003qos}&He, 2003 & 490&MINMIN & heuristic & limited & single & makespan & \no& \no& \no& \no& \no \\
% \cite{yu2005cost}&Yu, 2005 &443& MDP & heuristic & limited  & cost & \yes& \no& \no& \no &\no\\
\rowcolor{black!10}
\cite{yu2006scheduling}&Yu, 2006 &337 & GA   & makespan +cost& \no& \no &\no\\
\cite{kim2007dynamically}&Kim, 2007 &114 & SA  & makespan & \no& \no& \no\\
\rowcolor{black!10}
\cite{chen2009ant}&Chen, 2009 &293 & ACO   & makespan +reliability\tnote{*} & \yes& \no &\no\\
\cite{pandey2010particle}&Pandey, 2010 &519& PSO   & cost & \no& \no &\no\\
\rowcolor{black!10}
\cite{bittencourt2011hcoc}&Bittencourt, 2011 &181 & heuristic   & cost & \yes & \no & \no \\
\cite{fard2012multi}&Fard, 2012 &93 & heuristic  & makespan +cost&\no & \no &\no \\
\rowcolor{black!10}
\cite{abrishami2013deadline}&Abrishami, 2013 &264& heuristic   & deadline +cost&\no&\no&\no\\
\cite{rodriguez2014deadline}&Rodriguez, 2014 &181& PSO   & cost & \yes & \no & \no \\
\rowcolor{black!10}
\cite{tsai2014hyper}&Tsai, 2014 &57& SA+GA +PSO+ACO&makespan&\no&\no&\no\\
\cite{durillo2014multi}&Durillo, 2014 &45 & heuristic  & makespan +cost&\no & \no &\no \\
\rowcolor{black!10}
\cite{malawski2015algorithms}&Malawski, 2015 &230 & heuristic   & makespan +cost & \yes& \no &\no\\
% \cite{byun2011bts}&Byun, 2011 &38& BTS & heuristic & unlimited & single & cost\tnote{8} & \no & \yes &\no&\yes&\no\\
% \cite{zheng2006task}&Zheng, 2006 & 37&GSA& metaheuristic & limited& single & makespan & \no& \no& \no& \no& \no\\
% \rowcolor{Gray}
\cite{zhu2016evolutionary}&Zhu, 2016 &27 &  NSGA-II/SPEA2/ MOEAD  & makespan +cost   &\yes & \no & \no\\\bottomrule

\multicolumn{2}{c}{\bf This paper}  & ~ & sampling-based   & makespan +cost & \yes & \yes & \yes 
\\\\
\end{tabular}
\begin{tablenotes}
    % \item[1] Large workflow contains more than 100 tasks.
    % \item[2] Be able to make quick decisions corresponding to unexpected cloud environment changes during workflow execution.
    \item[*] Objectives were combined to one by a weight vector.           
\end{tablenotes}
\end{threeparttable}
\label{tab:relatedwork}
\end{table}


